Probability Measures for Numerical Solutions of Differential Equations

In this paper, we present a formal quantification of epistemic uncertainty induced by numerical solutions of ordinary and partial differential equation models. Numerical solutions of differential equations contain inherent uncertainties due to the finite dimensional approximation of an unknown and implicitly defined function. When statistically analysing models based on differential equations describing physical, or other naturally occurring, phenomena, it is therefore important to explicitly account for the uncertainty introduced by the numerical method. This enables objective determination of its importance relative to other uncertainties, such as those caused by data contaminated with noise or model error induced by missing physical or inadequate descriptors. To this end we show that a wide variety of existing solvers can be randomised, inducing a probability measure over the solutions of such differential equations. These measures exhibit contraction to a Dirac measure around the true unknown solution, where the rates of convergence are consistent with the underlying deterministic numerical method. Ordinary differential equations and elliptic partial differential equations are used to illustrate the approach to quantifying uncertainty in both the statistical analysis of the forward and inverse problems.

==> Litt_Rev.tex <==
% !TEX root = main.tex
\section{Literature Review}


\subsection{Literature Review}

Connections between probability and numerical analysis have
been understood and exploited for some time. The paper
\cite{diaconis1988bayesian} explains this connection in
the context of Bayesian statistics. The paper \cite{skilling}
demonstrated how numerical integration of differential
equations could be interpreted in a Bayesian fashion,
and this idea was converted into an operational methodology,
and consistency proofs given, in the paper \cite{chkr13}.
Furthermore, generalizations of the work in \cite{chkr13}  are emerging 
\cite{schober2014probabilistic}. The approach of \cite{chkr13}
builds a probabilistic structure around deterministic numerical
integration, which contains two sources of randomness: an overarching Gaussian
process structure, which can be used for implementation of the
methods in a framework familiar to researchers in machine learning,
and an internal randomization of the mean process, resulting
in different draws of the mean for each realization. Careful
analysis reveals that the outer Gaussian process structure does
not contain useful information about the uncertainty inherent
in the numerical method, because it does not interact with
the evaluations of the vector field which are generated
during the integration (this is the fact, familiar from
conjugate linear Gaussian models, that the posterior covariance
does not see the data). On the other hand the internal
randomization of the mean does interact with the
evaluations of the vector field and contains useful information
about uncertainty. The purpose of this paper is to build on this
observation to construct new probabilistic integration methods
for ODEs. Earlier work in the numerical analysis literature
in which randomization is used as part of the approximate
integration of ODEs includes \cite{coul99,sten95}. 




